Code Review Practices for Refactoring Changes: An Empirical Study on OpenStack

Modern code review is a widely used technique employed in both industrial and open-source projects to improve software quality, share knowledge, and ensure adherence to coding standards and guidelines. During code review, developers may discuss refactoring activities before merging code changes in the code base. To date, code review has been extensively studied to explore its general challenges, best practices and outcomes, and socio-technical aspects. However, little is known about how refactoring is being reviewed and what developers care about when they review refactored code. Hence, in this work, we present a quantitative and qualitative study to understand what are the main criteria developers rely on to develop a decision about accepting or rejecting a submitted refactored code, and what makes this process challenging. Through a case study of 11,010 refactoring and non-refactoring reviews spread across OpenStack open-source projects, we find that refactoring-related code reviews take significantly longer to be resolved in terms of code review efforts. Moreover, upon performing a thematic analysis on a significant sample of the refactoring code review discussions, we built a comprehensive taxonomy consisting of 28 refactoring review criteria. We envision our findings reaffirming the necessity of developing accurate and efficient tools and techniques that can assist developers in the review process in the presence of refactorings.

==> Tables/RQ1_statistics.tex <==
\begin{table}
  \centering
\caption{Results of Mann-Whitney U test and effect size for refactoring and non-refactoring code reviews.}
\label{Table:RQ1_statistical_test}
%\begin{sideways}
\begin{adjustbox}{width=0.5\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{llll}\hline
\toprule
\bfseries Metric &  \bfseries \textit{p}-value & \bfseries Cliff's delta ($\delta$)  \\
\midrule
Number of reviewers  &   \textbf{6.750458e-43} & small (0.15)
\\ 
Number of review comments  & \textbf{2.730193e-82} & small (0.22)
\\
Number of inline comments &  \textbf{2.066649e-98} & medium (0.33)
\\
Number of revisions &   \textbf{1.252695e-126} & small (0.3) 
  
\\
Number of changed files &   \textbf{6.006899e-190} & medium (0.33)

\\
Review duration  &   \textbf{2.572584e-66} & small (0.23)

\\
Length of discussion &   \textbf{6.966752e-42} & small (0.15)

\\
Length of description &   \textbf{4.071541e-41} & small (0.13)
  
\\ 
Code churn &   \textbf{0.000000e+00} &  large (0.64)

\\
\bottomrule
\end{tabular}
\end{adjustbox}
%\end{sideways}
\end{table}
